Characterization of a CMOS pixel sensor for charged particle tracking

A prototype of the CMOS pixel sensor named SUPIX-1 has been fabricated and tested in order to investigate the feasibility of a pixelated tracker for a proposed Higgs factory, namely, the Circular Electron-Positron Collider (CEPC). The sensor, taped out with a 180 nm CMOS Image Sensor (CIS) process, consists of nine different pixel arrays varying in pixel pitches, diode sizes and geometries in order to study the particle detection performance of enlarged pixels. The test was carried out with a Fe-55 radioactive source. Two soft X-ray peaks observed were used to calibrate the charge to voltage factor of the sensor. The pixel-wise equivalent noise charge, charge collection efficiency and signal-to-noise ratio were evaluated. A reconstruction method for clustering pixels of a signal has been developed and the cluster-wise performance was studied as well. The test results show that pixels with the area as large as of $21\mu$m$\times 84\mu$m have satisfactory noise level and charge collection performance, meeting gerenal requirements for a pixel sensor. This contribution demonstrates that the CMOS pixel sensor with enlarged pitches, using the CIS technology, can be used in tracking for upcoming collider detectors akin to the CEPC.

==> fit_results.tex <==
  \begin{tabular}{|c|c|c|c|c|c|}
    \hline
    Parameters & Crystal Ball & $\text{Gaussian}_\text{k-$\beta$}$ & Exponential & Gaussian 1 & Gaussian 2 \\
    \hline
     $\alpha$ & $0.9 \pm 0.1$ & - & - & - & - \\
     n & $0.04 \pm 0.02$ & - & - & - & -\\
     A & $610.4 \pm 10.7$ & $64.3 \pm 3.2$ & - & $1470.1 \pm 112.1$ & $1282.2 \pm 61.2$\\ 
     $\mu$ & $168.9 \pm 0.1$ & $185.4 \pm 0.3$ & - & $62.9 \pm 0.2$ & $84.5 \pm 1.7$\\
     $\sigma$ & $4.2 \pm 0.1$ & $4.0 \pm 0.2$ & - & $12.2 \pm 0.4$ & $21.8 \pm 0.8$\\
     C & - & - & $8.4 \pm 0.2$ & - & -\\
     Slope & - & - & $-0.1 \pm 0.01$ & - & -\\
     \hline
  \end{tabular}


==> table_result.tex <==
  \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
    \hline
    & \multicolumn{4}{c|}{pixel-wise} & \multicolumn{2}{c|}{cluster-wise} \\
    \hline
    Sector&CVF (\si{\mu V/e})& ENC (e)& CCE (\%) & SNR  & CCE (\%) & SNR \\
    \hline
    A0& 12.7$\pm$4.6 & 12.7$\pm$5.2 &	$39.1^{+20.2}_{-11.3}$ &	$52.4^{+28.9}_{-18.3}$ &	95.6$\pm$6.2& 	37.4$\pm$14.1\\
    \hline
    A2& 14.2$\pm$5.0 & 11.9$\pm$4.8 &	$31.7^{+14.4}_{-7.9}$ &	$48.9^{+24.3}_{-15.8}$ &	90.3$\pm$6.5& 	33.6$\pm$12.1\\
    \hline
    A5& 12.4$\pm$4.3 & 13.1$\pm$5.4 &	$27.5^{+25.7}_{-6.2}$ &	$35.7^{+34.2}_{-11.0}$ &	93.8$\pm$6.5& 	35.6$\pm$14.2\\
    \hline
    A7& 13.8$\pm$3.7 & 12.1$\pm$4.0 &	$30.4^{+28.8}_{-7.2}$ &	 $42.3^{+26.0}_{-13.1}$ &	96.8$\pm$5.4& 	42.6$\pm$18.6\\
    \hline
    A8& 13.3$\pm$4.9 & 12.4$\pm$5.2 &	$37.2^{+18.1}_{-6.6}$ &	$53.1^{+27.8}_{-14.0}$ &	92.4$\pm$6.1& 	40.7$\pm$16.8 \\
    
    \hline
  \end{tabular}

